Comparative Insights from 12 Machine Learning Models in Extracting Economic Ideology from Political Text

This study conducts a systematic assessment of the capabilities of 12 machine learning models and model variations in detecting economic ideology. As an evaluation benchmark, I use manifesto data spanning six elections in the United Kingdom and pre-annotated by expert and crowd coders. The analysis assesses the performance of several generative, fine-tuned, and zero-shot models at the granular and aggregate levels. The results show that generative models such as GPT-4o and Gemini 1.5 Flash consistently outperform other models against all benchmarks. However, they pose issues of accessibility and resource availability. Fine-tuning yielded competitive performance and offers a reliable alternative through domain-specific optimization. But its dependency on training data severely limits scalability. Zero-shot models consistently face difficulties with identifying signals of economic ideology, often resulting in negative associations with human coding. Using general knowledge for the domain-specific task of ideology scaling proved to be unreliable. Other key findings include considerable within-party variation, fine-tuning benefiting from larger training data, and zero-shot's sensitivity to prompt content. The assessments include the strengths and limitations of each model and derive best-practices for automated analyses of political content.

==> tabs2/9_compare_manif_optimize.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Tue Dec  3 19:55:43 2024
\begin{table}[ht]
\centering
\caption{Manifesto-level predicted economic ideology scores using fine-tuned POLITICS model at different sizes of the training set.} 
\label{tab2:manif_crowd_optimize}
\begingroup\footnotesize
\begin{tabular}{lrrrrrrr}
  \hline
Manifesto & Crowd Pos. & Experts Pos. & 1000 \nSentences & 900 \nSentences & 800 \nSentences & 700 \nSentences & 600 \nSentences \\ 
  \hdashline
Con 1987 & 0.19 & 0.37 & 0.87 & 1.13 & 1.07 & 1.09 & 0.73 \\ 
  Con 1992 & 0.20 & 0.33 & 0.91 & 1.16 & 1.08 & 1.11 & 0.71 \\ 
  Con 1997 & 0.22 & 0.33 & 0.82 & 1.06 & 1.01 & 1.04 & 0.77 \\ 
  Con 2001 & 0.26 & 0.51 & 0.93 & 1.16 & 1.13 & 1.11 & 0.82 \\ 
  Con 2005 & 0.37 & 0.36 & 0.87 & 1.12 & 1.08 & 1.04 & 0.80 \\ 
  Con 2010 & 0.11 & 0.22 & 0.85 & 1.09 & 1.08 & 1.06 & 0.81 \\ 
  Lab 1987 & -0.58 & -0.87 & 0.70 & 1.04 & 1.01 & 0.98 & 0.70 \\ 
  Lab 1992 & -0.49 & -0.57 & 0.70 & 0.97 & 0.96 & 0.97 & 0.66 \\ 
  Lab 1997 & -0.30 & -0.26 & 0.82 & 1.09 & 1.06 & 1.02 & 0.75 \\ 
  Lab 2001 & -0.45 & -0.43 & 0.68 & 0.91 & 0.90 & 0.91 & 0.63 \\ 
  Lab 2005 & -0.39 & -0.43 & 0.63 & 0.89 & 0.91 & 0.90 & 0.62 \\ 
  Lab 2010 & -0.24 & -0.33 & 0.67 & 0.92 & 0.94 & 0.92 & 0.62 \\ 
  LD 1987 & -0.32 & -0.40 & 0.77 & 1.01 & 0.98 & 1.00 & 0.67 \\ 
  LD 1992 & -0.35 & -0.38 & 0.74 & 1.01 & 0.99 & 1.00 & 0.64 \\ 
  LD 1997 & -0.27 & -0.44 & 0.72 & 0.98 & 0.96 & 0.94 & 0.71 \\ 
  LD 2001 & -0.36 & -0.43 & 0.76 & 0.98 & 0.97 & 0.99 & 0.69 \\ 
  LD 2005 & -0.18 & -0.26 & 0.79 & 1.03 & 1.03 & 1.06 & 0.76 \\ 
  LD 2010 & -0.27 & -0.31 & 0.73 & 1.03 & 1.03 & 1.04 & 0.78 \\ 
   \hline
\end{tabular}
\endgroup
\end{table}

